Even your Teacher Needs Guidance: Ground-Truth Targets Dampen Regularization Imposed by Self-Distillation

Knowledge distillation is classically a procedure where a neural network is trained on the output of another network along with the original targets in order to transfer knowledge between the architectures. The special case of self-distillation, where the network architectures are identical, has been observed to improve generalization accuracy. In this paper, we consider an iterative variant of self-distillation in a kernel regression setting, in which successive steps incorporate both model outputs and the ground-truth targets. This allows us to provide the first theoretical results on the importance of using the weighted ground-truth targets in self-distillation. Our focus is on fitting nonlinear functions to training data with a weighted mean square error objective function suitable for distillation, subject to $\ell_2$ regularization of the model parameters. We show that any such function obtained with self-distillation can be calculated directly as a function of the initial fit, and that infinite distillation steps yields the same optimization problem as the original with amplified regularization. Furthermore, we provide a closed form solution for the optimal choice of weighting parameter at each step, and show how to efficiently estimate this weighting parameter for deep learning and significantly reduce the computational requirements compared to a grid search.

==> Even your Teacher Needs Guidance (arXiv)/constrained.tex <==
\section{Connections to Constrained Optimization Problem}\label{app:mobahi}
The setup investigated in this paper is the unconstrained optimization problem presented in \eqref{eq:unconstrained_optimization}, but some of the results can easily be extended to a constrained optimization problem, with a general regularization functional in Hilbert spaces, namely the natural extension of the setup proposed by \citet{mobahi2020selfdistillation}. For the rest of this section we assume $\alpha^{(2)} = \dots = \alpha^{(\tau)} = \alpha$. \citet{mobahi2020selfdistillation} propose to solve the problem
\begin{align}\label{eq:mohabi}
    f^{(\tau)} \eqdef \argmin_{f \in \F} \int_\mathcal{X} \int_\mathcal{X} u(\bm{x}, \bm{x}') f(\bm{x}) f(\bm{x}') d\bm{x} d\bm{x}' \quad \text{s.t.} \quad \frac{1}{N} \sum_{n=1}^{N} \left(f(\bm{x}_n) - y_n \right)^2 \leq \varepsilon,
\end{align}
where $\varepsilon > 0$ is a desired loss tolerance, $\tau \geq 1$, $f^{(0)} (\bm{x}_n) = y_n$ for $n=1, \dots, N$,  and $u$ being symmetric and such that $\forall f \in \mathcal{F}$\footnote{For a given $u$ the function space $\mathcal{F}$ is the space of functions $f$ for which the double integral in \eqref{eq:mohabi} is bounded.} the double integral is greater than or equal to $0$ with equality only when $f(x) = 0$. See \citet{mobahi2020selfdistillation} for details.

The natural extension of this problem is to include ground-truth labels, and solve the weighted problem
\begin{align}\label{eq:mohabi_extension}
    &f^{(\tau)} = \argmin_{f \in \F} \int_\mathcal{X} \int_\mathcal{X} u(\bm{x}, \bm{x}') f(\bm{x}) f(\bm{x}') d\bm{x} d\bm{x}' \\ \text{s.t.} \quad &\frac{\alpha}{N} \sum_{n=1}^{N} \left(f(\bm{x}_n) - y_n \right)^2 + \frac{1-\alpha}{N}\sum_{n=1}^{N} \left( f(\bm{x}_n) - f^{(\tau-1)}(\bm{x}_n) \right)^2 \leq \varepsilon,
\end{align}
for $\tau \geq 1$, where $\alpha \in [0,1]$ and $f^{(0)} (\bm{x}_n) = y_n$ for $n=1, \dots, N$. In \citet{mobahi2020selfdistillation}, $\alpha = 0$, and this problem completely ignores the ground truth data after the first model fit, and it is easy to see that consecutive self-fits will be penalized increasingly stronger, and eventually collapse to zero, whenever $\frac{1}{N} \sum_{n=1}^{N} \left(f(\bm{x}_n) - y_n \right)^2 \leq \varepsilon$. The case $\alpha = 1$, corresponds to fitting to the ground-truth at each iteration, and do not benefit from distillation, and thus is without interest here.

\subsection{Collapsing and converging conditions}\label{sec:collapsing_converging}
The regularization functional of \eqref{eq:mohabi_extension}, is clearly minimized by $f_t(\bm{x}) = 0$, but in order for this to be a solution for some $\tau \geq 1$, it must hold that
\begin{align*}
    \frac{\alpha}{N}\norm{\bm{y}}_2^2 + \frac{1-\alpha}{N}\norm{\bm{y}^{(\tau-1)}}_2^2 \leq \varepsilon,
\end{align*}
where we use the notation that $\bm{y}^{(\tau)} = (f^{(\tau)}(\bm{x}_1), \dots, f^{(\tau)}(\bm{x}_N))^T$ and $\bm{y} = (y_1, \dots, y_N)$. For $\tau = 1$, this amounts to $\frac{1}{N}\norm{\bm{y}}_2^2 \leq \varepsilon$, and for $\tau > 1$
\begin{align}\label{eq:collapse_condition}
    \frac{1-\alpha}{N}\norm{\bm{y}^{(\tau-1)}}_2^2 \leq \varepsilon - \frac{\alpha}{N}\norm{\bm{y}}_2^2.
\end{align}
But since the l.h.s. is non-negative, it is required that $\frac{\alpha}{N}\norm{\bm{y}}_2^2 \leq \varepsilon$ in order for $f^{(\tau)}(\bm{x}) = 0$ to be a solution. Hence, we can construct the following settings, that determine the behavior of the solutions:
\begin{enumerate}
    \item $\frac{1}{N}\norm{\bm{y}}_2^2 \in \left[0, \varepsilon\right] \implies \norm{\bm{y}^{(\tau)}}_2 = 0 ~\forall \tau \geq 1,$ \hfill (Collapsed solution)
    \item $\frac{1}{N}\norm{\bm{y}}_2^2 \in \left(\varepsilon, \frac{\varepsilon}{\alpha}\right] \implies \exists \underline{\tau} \geq 1$ such that $\begin{cases} \norm{\bm{y}^{(\tau)}}_2 > 0 &\forall \tau < \underline{\tau}, \\ \norm{\bm{y}^{(\tau)}}_2 = 0 &\forall \tau \geq \underline{\tau},\end{cases}$ \hfill (Converging to collapsed solution)
    \item $\frac{1}{N}\norm{\bm{y}}_2^2 \in \left(\frac{\varepsilon}{\alpha}, \infty\right) \implies \norm{\bm{y}^{(\tau)}}_2 > 0 ~\forall \tau \geq 1$. \hfill (Converging to non-collapsed solution)
\end{enumerate}
If we let $\alpha \to 0$ the interval $\left(\varepsilon, \frac{\varepsilon}{\alpha}\right]$ effectively becomes $\left(\varepsilon, \infty\right)$, and any solution will collapse at some point \citep{mobahi2020selfdistillation}. Analogously, if we let $\alpha \to 1$, the interval $(\varepsilon, \frac{\varepsilon}{\alpha}]$ effectively becomes empty, and all non-collapsed solutions will converge to a non-zero solution. Hence, if $\alpha > 0$, one can obtain non-collapsing convergence with infinite iterations. Furthermore, if we let $\varepsilon \to 0$, then $[0,\varepsilon]$ and $(\varepsilon, \frac{\varepsilon}{\alpha}]$ will practically collapse to empty intervals, and we will always obtain convergence to non-collapsing solutions, which will correspond to an interpolating solution.
For the remainder we assume $\alpha \in (0, 1)$, since the boundary cases are covered in \citet{mobahi2020selfdistillation} ($\alpha = 0$) or is without interest ($\alpha = 1$). Furthermore, we assume that $\norm{\by}_2 > \sqrt{N\varepsilon}$ to avoid a collapsed solution from the beginning. Utilizing the Karush-Kuhn-Tucker (KKT) conditions for this problem, we can rephrase our optimization problem as
\begin{align}\label{eq:problem_mobahi}
    f^{(\tau)} &= \argmin_{f \in \F} \frac{\alpha}{N}\sum_{n=1}^{N} \left(f(\bm{x}_n) - y_n \right)^2 + \frac{1-\alpha}{N}\sum_{n=1}^{N} \left( f(\bm{x}_n) - f^{(\tau-1)}(\bm{x}_n) \right)^2 \nonumber \\ 
    &+ \lambda_\tau \int_\mathcal{X} \int_\mathcal{X} u(\bm{x}, \bm{x}') f(\bm{x}) f(\bm{x}') d\bm{x} d\bm{x}',
\end{align}
where $\lambda_{\tau} \geq 0$. For suitably chosen $\lambda_{\tau}$, one can show that $f^{(\tau)}$ is an optimal solution to our problem\footnote{See \citet{mobahi2020selfdistillation} for a detailed argument.}.

\subsection{Extending our results}
By direct calculations similar to those of \citet{mobahi2020selfdistillation} one can obtain the closed form solution of \eqref{eq:problem_mobahi}, but first we will repeat some definitions from \citet{mobahi2020selfdistillation}. Let the Green's Function $g(x,t)$ be such that $\int_{\mathcal{X}} u(x, x') g(x', t) dx' = \delta(x - t)$, where $\delta$ is the Dirac delta, and let $[\bG]_{j,k} = \frac{1}{N} g(\bx_j, \bx_k)$ and $[\bg(\bx)]_k = \frac{1}{N} g(\bx, \bx_k)$, where $\bG$ is a matrix and $\bg(\bx)$ a vector dependent on $\bx$.
Now we can present the proposition.
\begin{proposition}\label{prop:solution}
For any $\tau \geq 1$, the problem \eqref{eq:problem_mobahi} has a solution of the form
\begin{align*}
    \by^{(\tau)} = \bg(\bx)^\trans \left(\bG +  \lambda_{\tau}\bI\right)^{-1}(\alpha \by + (1-\alpha)\by^{(\tau-1)}),
\end{align*}
where $\by^{(0)} \eqdef \by$.
\end{proposition}

Since $\bG$ is positive semi-definite, we can decompose it as $\bG = \bV \bD \bV^\trans$. Define $\bB^{(0)} \eqdef \bI$, then for $\tau \geq 1$, we have that $\by^{(\tau)} = \bV \bB^{(\tau)} \bV^\trans \by$, where we set
\begin{align*}
    \bB^{(\tau)} &\eqdef \frac{\alpha}{1-\alpha}\sum_{i=1}^{\tau-1} \left(1-\alpha\right)^{\tau-i} \prod_{j=i}^{\tau-1} \bA^{(j+1)} + \left(1-\alpha\right)^{\tau-1}\prod_{j=1}^\tau \bA^{(j)}, \\
    \bA^{(\tau)} &\eqdef \bD(\bD + \lambda_{\tau} \bI)^{\inv}.
\end{align*}

By equivalent calculations as those of Lemma \ref{lem:recurrent_B}, we have that
\begin{align*}
    \bB^{(\tau)} = \bA^{(\tau)}((1-\alpha)\bB^{(\tau-1)} + \alpha \bI_N) \quad \forall \tau \geq 1,
\end{align*}
and we can now formulate the following theorem, similar to Theorem \ref{thm:B_sparsification}.

\begin{theorem}
For any pair of diagonals of $\bD$, i.e. $d_k$ and $d_j$, where $d_k > d_j$, we have that for all $\tau \geq 1$ and for $\alpha \in (0, 1)$, then
\begin{align}
    &\mathrm{sign}\left(\frac{[\bB^{(\tau)}]_{k,k}}{[\bB^{(\tau)}]_{j,j}} - \frac{[\bB^{(\tau-1)}]_{k,k}}{[\bB^{(\tau-1)}]_{j,j}} \right) \\
    &= \mathrm{sign}\left(\left( \left(\frac{[\bB^{(\tau-1)}]_{k,k}}{[\bB^{(\tau-1)}]_{j,j}} - \frac{[\bA^{(\tau)}]_{k,k}}{[\bA^{(\tau)}]_{j,j}} \right) \frac{[\bA^{(\tau)}]_{j,j}}{[\bB^{(\tau-1)}]_{k,k} ([\bA^{(\tau)}]_{k,k} - [\bA^{(\tau)}]_{j,j})} + 1\right)^\inv - \alpha \right).
\end{align}
\end{theorem}
\begin{proof}
The proof follows by analogous calculations to the proof of Theorem \ref{thm:B_sparsification}.
\end{proof}
For the case $\alpha = 1$, the results is identical to Theorem \ref{thm:B_sparsification}, since no distillation is actually performed. However, the case $\alpha = 0$ is more involved and we refer the reader to \citet{mobahi2020selfdistillation} for the treatment of this case, since our setup is identical to that of \citet{mobahi2020selfdistillation} when $\alpha = 0$.

Finally, due to the dependency of $\lambda_{\tau}$ on the solution from the previous step of distillation in this constrained optimization problem, we are unable to obtain a simple recurrent expression as \eqref{eq:recurrent_y} and a limiting solution as in Theorem \ref{thm:kernel_limit}. However, by the results in Section \ref{sec:collapsing_converging}, we can determine, from the norm of the targets, whether the solution collapses or not.

==> Even your Teacher Needs Guidance (arXiv)/experiments.tex <==

\section{Experiments}\label{sec:experiments}
In the following we show empirical results of performing a simple self-distillation procedure with deep neural networks with varying choices of $\alpha$ to investigate the large scale effects. The experiments are adapted from \citet{mobahi2020selfdistillation} with the additional introduction of the $\alpha$-parameter. For stronger baselines of the possible performance gains from self-distillation see e.g. \citet{furlanello2018born, Tian2020RethinkingNeed, Ahn2019VariationalTransfer, Yang2018KnowledgeStudents}.
The following sections provide additional details to that of Section \ref{sec:optimal_alpha_DL}.

\subsection{Experimental Setup}
We perform self-distillation with ResNet-50 \citep{He2016DeepRecognition} networks on CIFAR-10 \citep{Krizhevsky2009LearningImages}, with minor pre-processing and augmentations.\footnote{Training: We randomly flip an image horizontally with probability $\frac{1}{2}$, followed by a random $32 \times 32$ crop of the $40 \times 40$ zero padded image. Finally we normalize the image to have mean $0$ and standard deviation $1$. Validation: We normalize the image with the empirical mean and standard deviation from the training data.} The model is initialized randomly at each step\footnote{Note, we initialize the models equally across all $\alpha$ for one experiment, but alter the seed for initialization between experiments.} and trained as described in Section \ref{sec:optimal_alpha_DL} with either estimated optimal parameters, $\hat{\alpha}^{(\tau)}$, or fixed $\alpha$ for all steps. We use Adam optimizer with a learning rate of $10^{-4}$, $\ell_2$ regularization with regularization coefficient $10^{-4}$, and train on the full $50000$ training images and validate our generalization performance on the $10000$ test images. We use the weights from the last step of optimization at each distillation step for the next step, irrespective of whether a better model occurred earlier in the training. Our models are trained for a fixed $75$ epochs, which does not allow our models to overfit the training data, which is important for our models to be suitable for distillation procedures \citep{Dong2019DistillationNetwork}. The experiments are performed on a single Nvidia Tesla V100 16GB GPU with the PyTorch Lightning framework \citep{Falcon2019PyTorchLightning}.

\subsection{Results}
We repeat our experiment $4$ times and illustrate the mean, minimum and maximum at each distillation step in Figure \ref{fig:optimal_resnet50_by_step}. Each experiment is $11$ chains of distillation steps, corresponding to $\alpha \in \{0.0, 0.1, \dots, 0.9\}$, with the first model initialized identically across all chains. The accuracy reported at the $\tau$'th step is based on comparing the training and validation predictions, $\bY^{(\tau)}$ and $f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})$ with the original training and validation targets; $\bY$ and $\tilde{\bY}$.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.44\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/resnet50_optimal_train.pdf}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.515\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/resnet50_optimal_val.pdf}
    \end{subfigure}
    \caption{(Identical to Figure \ref{fig:optimal_resnet50_by_step}) Training and validation accuracy for five distillation steps with ResNet-50 models on CIFAR-10. Comparing fixed $\alpha^{(t)}$ for $t=2\dots,\tau$ and estimating optimal weight with $\hat{\alpha}^{(t)}$ at each step. The experiment is repeated four times and the mean (and max/min in shaded) is reported.}
\end{figure}

The theory introduced in Section \ref{sec:main_results} suggests that self-distillation corresponds to a progressively amplified regularization of the solution, and larger $\alpha$ dampens the amount of regularization imposed by the procedure more than small values of $\alpha$. Thus, for small $\alpha$ we expect the training accuracy to decrease with each distillation, but for larger $\alpha$ we might experience an increase in training accuracy, due to additional training iterations and a sufficient amount of ground-truth target information being kept in the optimization problem, which could prove beneficial. However, depending on the need for increased regularization, we expect the validation accuracy to increase for some $\alpha$, and possibly decrease for $\alpha$ values either too small or too large. The above properties are observed in Figure \ref{fig:optimal_resnet50_by_step}, where $\alpha \leq 0.4$ generally overregularize the solution, and performance drops with distillation steps. For $\alpha > 0.4$ the performance generally improves with distillation, but for $\alpha$ close to one, the gains reduce, and a suitably balanced $\alpha$ for this experiment would be in $[0.5, 0.7]$. This aligns well with the optimal $\hat{\alpha}^{(\tau)}$ estimated at approx. $0.6$ for each step of self-distillation.

==> Even your Teacher Needs Guidance (arXiv)/ntk.tex <==
\section{Connection to Neural Networks}\label{sec:ntk}
This paper theoretically investigates self-distillation of kernel ridge regression models, but distillation procedures are more commonly used in a deep learning setting. However, recent research in the over-parameterized regime has shown great progress and connected wide neural networks with kernel ridge regression using the Neural Tangent Kernel (NTK) \citep{Lee2019WideDescent, Lee2020GeneralizedNetworks, Hu2019SimpleGuarantee}. The following is a brief and informal connection between kernel ridge regression and wide\footnote{Note, we refer to width as the number of hidden nodes in a fully connected neural network or channels in a convolutional neural network.} neural networks, motivating our problem setup and approach to estimate $\hat{\alpha}^{(\tau)}$ in Section \ref{sec:optimal_alpha_DL}.

Consider a neural network with scalar output $\nn(\bx, \btheta) \in \R$, where $\btheta(t) \in \R^D$ is the vector of all network parameters at training iteration $t \geq 0$, and $\bx \in \R^d$ some input. We consider the case where we use gradient descent on the MSE objective, $\L(\btheta) = \frac{1}{2}\sum_{i=1}^n (\nn(\bx_i, \btheta) - y_i)^2$ over some training dataset $\D_\mathrm{train} \subseteq \R^d \times \R$. Consider the first-order Taylor-expansion of $\nn(\bx, \btheta)$ w.r.t its parameters at initialization, $\btheta(0)$,
\begin{align}\label{eq:NTK_approx}
    \nn(\bx, \btheta) \approx \nn(\bx, \btheta(0)) + \langle\nabla_{\btheta} \nn(\bx, \btheta(0)), \btheta - \btheta(0)\rangle
\end{align}
where $\nn(\bx, \btheta(0))$ and $\nabla_{\btheta} \nn(\bx, \btheta(0))$ are constants w.r.t. $\btheta$. For sufficiently wide networks, \eqref{eq:NTK_approx} holds, and we say that we are in the \emph{(NTK) regime} \citep{Arora2019OnNet, Lee2019WideDescent}. Now, let $\varphi(\bx) \eqdef \nabla_{\btheta} \nn(\bx, \btheta(0))$ for any $\bx \in \R^d$, and denote the random kernel $\kappa(\bx_i, \bx_j) \eqdef \langle\varphi(\bx_i), \varphi(\bx_j)\rangle$ for any $\bx_i, \bx_j \in \R^d$ \citep{Jacot2018NeuralNetworks}. For sufficiently wide networks, the random kernel converges to a deterministic kernel, and since the r.h.s. of \eqref{eq:NTK_approx} is linear, one can show that minimizing $\L$ with gradient descent leads to the solution of the kernel regression problem, with the NTK; $\bx \mapsto \kappa(\bx, \bX)^\trans \kappa(\bX, \bX)^\inv \by$, where $\bX \in \R^{n \times d}$ is the matrix of training inputs, and $\by \in \R^n$ the vector of training targets \citep{Arora2019OnNet, Lee2019WideDescent}. It has been shown that when minimizing the $\ell_2$-regularized MSE loss, the solution becomes the kernel ridge regression solution \citep{Lee2020GeneralizedNetworks}.

The connections between neural networks and kernel ridge regressions in knowledge distillation settings have, to the best of our knowledge, not been explicitly investigated yet, but we hope that the results of this paper will improve the understanding of self-distillation of neural networks once such a connection is made rigorously.

==> Even your Teacher Needs Guidance (arXiv)/preamble.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Packages for template
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors

\usepackage{graphicx}           % allows for minipage figures
\usepackage{natbib}             % better citations
\usepackage{amsmath}            % general math package
\usepackage{amssymb}            % math symbols
\usepackage{amsthm}             % theorems, propositions etc.
\usepackage{enumitem}           % pretty lists
\usepackage{parskip}            % tweak paragraph skipping (blank line = paragraph)
\usepackage{bm}                 % bold math
\usepackage{dsfont}             % for indicator font
\usepackage{caption}            % for subfigures
\usepackage{subcaption}         % for subfigures
\usepackage[ruled]{algorithm2e} %linesnumbered
\newcommand{\nosemic}{\SetEndCharOfAlgoLine{\relax}}% Drop semi-colon ;
\newcommand{\dosemic}{\SetEndCharOfAlgoLine{\string;}}% Reinstate
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\usepackage{wrapfig}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Custom math
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathcal{F}}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}

\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand{\bbeta}{\bm{\beta}}
\newcommand{\bgamma}{\bm{\gamma}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bomega}{\bm{\omega}}
\newcommand\eqdef{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}} % the eqdef command for defining equalities
\newcommand{\trans}{{\intercal}}
\newcommand{\inv}{{-1}}
\newcommand{\nn}{f_{\mathrm{nn}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}

\newcommand\bA{\mathbf{A}}
\newcommand\bB{\mathbf{B}}
\newcommand\bC{\mathbf{C}}
\newcommand\bD{\mathbf{D}}
\newcommand\bE{\mathbf{E}}
\newcommand\bF{\mathbf{F}}
\newcommand\bG{\mathbf{G}}
\newcommand\bH{\mathbf{H}}
\newcommand\bI{\mathbf{I}}
\newcommand\bJ{\mathbf{J}}
\newcommand\bK{\mathbf{K}}
\newcommand\bL{\mathbf{L}}
\newcommand\bM{\mathbf{M}}
\newcommand\bN{\mathbf{N}}
\newcommand\bO{\mathbf{O}}
\newcommand\bP{\mathbf{P}}
\newcommand\bQ{\mathbf{Q}}
\newcommand\bR{\mathbf{R}}
\newcommand\bS{\mathbf{S}}
\newcommand\bT{\mathbf{T}}
\newcommand\bU{\mathbf{U}}
\newcommand\bV{\mathbf{V}}
\newcommand\bW{\mathbf{W}}
\newcommand\bX{\mathbf{X}}
\newcommand\bY{\mathbf{Y}}
\newcommand\bZ{\mathbf{Z}}

\newcommand\ba{\mathbf{a}}
\newcommand\bb{\mathbf{b}}
\newcommand\bc{\mathbf{c}}
\newcommand\bd{\mathbf{d}}
\newcommand\be{\mathbf{e}}
\newcommand\bbf{\mathbf{f}} %bold f can't be bf
\newcommand\bg{\mathbf{g}}
\newcommand\bh{\mathbf{h}}
\newcommand\bi{\mathbf{i}}
\newcommand\bj{\mathbf{j}}
\newcommand\bk{\mathbf{k}}
\newcommand\bl{\mathbf{l}}
\newcommand\bbm{\mathbf{m}} %bold m can't be bm
\newcommand\bn{\mathbf{n}}
\newcommand\bo{\mathbf{o}}
\newcommand\bp{\mathbf{p}}
\newcommand\bq{\mathbf{q}}
\newcommand\br{\mathbf{r}}
\newcommand\bs{\mathbf{s}}
\newcommand\bt{\mathbf{t}}
\newcommand\bu{\mathbf{u}}
\newcommand\bx{\mathbf{x}}
\newcommand\bv{\mathbf{v}}
\newcommand\bw{\mathbf{w}}
\newcommand\by{\mathbf{y}}
\newcommand\bz{\mathbf{z}}

==> Even your Teacher Needs Guidance (arXiv)/proofs.tex <==
\section{Proofs}\label{sec:proofs}
This section includes all proofs referenced in the main part of the paper, along with the associated theorems and lemmas for completeness.

\begin{theorem}
Let $\by^{(\tau)}, \hat{\bbeta}^{(\tau)}$, and $f(\cdot, \hat{\bbeta}^{(\tau)})$ be defined as above. Fix $\alpha^{(2)}, \dots, \alpha^{(\tau)} \in [0, 1)$, and let $\eta(i, \tau) \eqdef \prod_{j=i}^{\tau} \left(1-\alpha^{(j)} \right)$, then for $\tau \geq 1$, we have that
\begin{align*}
    &\by^{(\tau)} = \left( \sum_{i=2}^{\tau} \alpha^{(i)} \eta(i+1, \tau) \left(\bK\left(\bK + \lambda \bI_n\right)^{-1}\right)^{\tau-i+1} + \eta(2, \tau)\left(\bK\left(\bK + \lambda \bI_n\right)^{-1}\right)^{\tau} \right) \by,\\
    &f(\bx, \hat{\bbeta}^{(\tau)}) = \alpha^{(\tau)} f(\bx, \hat{\bbeta}^{(1)}) + (1-\alpha^{(\tau)})f(\bx, \hat{\bbeta}^{(\tau)}_{\alpha=0})
\end{align*}
for any $\bx \in \R^{d}$, where $\hat{\bbeta}^{(\tau)}_{\alpha=0}$ is the minimizer in \eqref{eq:beta_minimizer} with $\alpha^{(\tau)} = 0$.
\end{theorem}
\begin{proof}
We prove the theorem by induction, where we let $\tilde{\bK} \eqdef \bK(\bK + \lambda\bI_n)^\inv$. For $\tau = 1$, the result hold trivially, and thus, assume it hold for $\tau = t$. Since $\bbeta^{(t+1)} = \varphi(\bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\alpha^{(t+1)}\by + (1-\alpha^{(t+1)})\by^{(t)}\right)$ we have that
\begin{align*}
    \by^{(t+1)} &= \varphi(\bX)\varphi(\bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\alpha^{(t+1)}\by + (1-\alpha^{(t+1)})\by^{(t)}\right) \\
    &= \alpha^{(t+1)} \tilde{\bK} \by + (1-\alpha^{(t+1)})\tilde{\bK} \left( \sum_{i=2}^{t} \alpha^{(i)} \eta(i+1, t) \tilde{\bK}^{t-i+1} + \eta(2, t)\tilde{\bK}^{t} \right) \by \\
    &= \alpha^{(t+1)} \tilde{\bK} \by + \left( \sum_{i=2}^{t} \alpha^{(i)} \eta(i+1, t+1) \tilde{\bK}^{(t+1)-i+1} + \eta(2, t+1)\tilde{\bK}^{t+1} \right) \by \\
    &= \left( \sum_{i=2}^{t+1} \alpha^{(i)} \eta(i+1, t+1) \tilde{\bK}^{(t+1)-i+1} + \eta(2, t+1)\tilde{\bK}^{t+1} \right) \by
\end{align*}
which finalizes our induction proof for the first part. For the second part, note that it also holds trivially for $\tau = 1$. Thus assume, it holds for $\tau = t$, then by direct manipulations
\begin{align*}
    f(\bx, \bbeta^{(t+1)}) &= \kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\alpha^{(t+1)}\by + (1-\alpha^{(t+1)})\by^{(t)} \right) \\
    &= \alpha^{(t+1)} f(\bx, \bbeta^{(1)}) + (1-\alpha^{(t+1)})\kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv \by^{(t)} \\
    &= \alpha^{(t+1)} f(\bx, \bbeta^{(1)}) + (1-\alpha^{(t+1)})f(\bx, \hat{\bbeta}^{(t+1)}_{\alpha=0}),
\end{align*}
where we let $\hat{\bbeta}^{(t+1)}_{\alpha=0}$ denote the minimizer \eqref{eq:beta_minimizer} with $\alpha^{(t+1)} = 0$; i.e. minimizing the classical kernel ridge regression problem with targets $\by^{(t)}$.
\end{proof}

\begin{lemma}
Let $\bB^{(\tau)}$, and $\bA$ be defined as above, and let $\bB^{(0)} \eqdef \bI$. Then we can express $\bB^{(\tau)}$ recursively as
\begin{align*}
    \bB^{(\tau)} = \bA\left((1-\alpha^{(\tau)})\bB^{(\tau-1)} + \alpha^{(\tau)} \bI_n\right),
\end{align*}
and $[\bB^{(\tau)}]_{k,k} \in [0,1]$ is (strictly) decreasing in $\tau$ for all $k \in [n]$ and $\tau \geq 1$ if $\alpha^{(2)} = \dots = \alpha^{(\tau)} = \alpha$.
\end{lemma}
\begin{proof}
The case, $\tau = 1$, is easy to verify, and we assume the claim holds for $\tau = t$. Then note that
\begin{align*}
    \bA\left((1-\alpha^{(t+1)})\bB^{(t)} + \alpha^{(t+1)} \bI_n \right) &= \sum_{i=2}^{t} \alpha^{(i)} \eta(i+1, t+1) \bA^{(t+1)-i+1} + \eta(2, t+1)\bA^{t+1} + \alpha^{(t+1)}\bA \\
    &= \sum_{i=2}^{t+1} \alpha^{(i)} \eta(i+1, t+1) \bA^{(t+1)-i+1} + \eta(2, t+1)\bA^{t+1} \\
    &= \bB^{(t+1)},
\end{align*}
finalizing the induction proof. Now, assume $\alpha^{(2)} = \dots = \alpha^{(\tau)} = \alpha$ and note that for any $k$ and $\tau \geq 1$, then
\begin{align*}
    [\bA]_k \left((1-\alpha)[\bB^{(\tau-1)}]_{k,k} + \alpha\right) = [\bB^{(\tau)}]_{k,k} \leq [\bB^{(\tau-1)}]_{k,k} = [\bA]_k \left((1-\alpha)[\bB^{(\tau-2)}]_{k,k} + \alpha\right),
\end{align*}
if and only if $[\bB^{(\tau-1)}]_{k,k} \leq [\bB^{(\tau-2)}]_{k,k}$, and iteratively, if and only if $[\bB^{(1)}]_{k,k} \leq [\bB^{(0)}]_{k,k}$. The latter is indeed true, since $\bB^{(1)} = \bA$, and finally, $\bA = \bI_n$ if and only if $\lambda = 0$.
%Furthermore, let $k \in [n]$, then since $[\bA]_{k,k} \in [0,1]$, we have that $[\bB^{(1)}]_{k,k} \in [0,1]$, and $[\bB^{(\tau)}]_{k,k} \leq [\bA]_{k,k}$ for any $\tau \geq 1$ which yield that $[\bB^{(\tau+1)}]_{k,k} \leq (1-\alpha)[\bA^{2}]_{k,k} + \alpha [\bA]_{k,k} \leq [\bA]_{k,k} \in [0,1]$, and we are done.
\end{proof}


\begin{theorem}
Assume $\alpha^{(2)} = \dots = \alpha^{(\tau)} = \alpha$. Then, for any pair of diagonals of $\bD$, i.e. $d_k$ and $d_j$, where $d_k > d_j$, we have that for all $\tau \geq 1$,
\begin{align*}
    \frac{[\bB^{(\tau)}]_{k,k}}{[\bB^{(\tau)}]_{j,j}} &= \begin{cases} \frac{1 + \frac{\lambda}{d_j}}{1 + \frac{\lambda}{d_k}}, &\text{for } \alpha = 1, \\ \left(\frac{1 + \frac{\lambda}{d_j}}{1 + \frac{\lambda}{d_k}}\right)^\tau, &\text{for } \alpha = 0, \end{cases}
\end{align*}
and if we let $\mathrm{sgn}(\cdot)$ denote the sign function, i.e.
\begin{align*}
    \mathrm{sgn}(x) \eqdef \begin{cases} \;1 &\text{if} \quad x > 0 \\ \;0 &\text{if} \quad x = 0 \\ -1 &\text{if} \quad x < 0\end{cases},
\end{align*}
then for $\alpha \in (0, 1)$ we have that
\begin{align*}
    &\mathrm{sgn}\left(\frac{[\bB^{(\tau)}]_{k,k}}{[\bB^{(\tau)}]_{j,j}} - \frac{[\bB^{(\tau-1)}]_{k,k}}{[\bB^{(\tau-1)}]_{j,j}} \right) \nonumber\\
    &\quad= \mathrm{sgn}\left(\left( \left(\frac{[\bB^{(\tau-1)}]_{k,k}}{[\bB^{(\tau-1)}]_{j,j}} - \frac{[\bA]_{k,k}}{[\bA]_{j,j}} \right)\frac{[\bA]_{j,j}}{[\bB^{(\tau-1)}]_{k,k} ([\bA]_{k,k} - [\bA]_{j,j})} + 1\right)^\inv - \alpha \right).
\end{align*}
\end{theorem}
\begin{proof}
First note that
\begin{align*}
    \frac{[\bA]_{k,k}}{[\bA]_{j,j}} = \frac{\frac{d_k}{d_k + \lambda}}{\frac{d_j}{d_j + \lambda}} = \frac{1 + \frac{\lambda}{d_j}}{1 + \frac{\lambda}{d_k}},
\end{align*}
and for $\alpha = 1$, \eqref{eq:recurrent_B} amounts to $\bB^{(\tau)} = \bA$, which gives the first result. For $\alpha = 0$, \eqref{eq:recurrent_B} amounts to $\bB^{(\tau)} = \bA^{\tau}$, and the second result follows. For the remainder we denote $[\bB^{(\tau-1)}]_{k,k}$ by $\bB_k$ and $[\bA]_{k,k}$ by $\bA_k$ to simplify notation. We investigate the case where both r.h.s. and l.h.s. equals zero. Thus, for $\alpha \in (0, 1)$, we observe that if
\begin{align*}
    \frac{\bB_k}{\bB_j} &= \frac{\bA_k}{\bA_j} \frac{(1-\alpha)\bB_k + \alpha}{(1-\alpha)\bB_j + \alpha} = \frac{\bA_k}{\bA_j}\frac{\frac{1-\alpha}{\alpha} \bB_k + 1}{\frac{1-\alpha}{\alpha}\bB_j + 1},
\end{align*}
then we have that
\begin{align*}
    \bB_j &= \frac{1}{\frac{\bA_k}{\bA_j}\left(\frac{\frac{1-\alpha}{\alpha}\bB_k + 1}{\bB_k}\right) - \frac{1-\alpha}{\alpha}} = \frac{\bB_k}{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right) - \frac{1-\alpha}{\alpha}\bB_k} \\
    \frac{1-\alpha}{\alpha}\bB_j + 1 &= \frac{\frac{1-\alpha}{\alpha}\bB_k}{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right) - \frac{1-\alpha}{\alpha}\bB_k} + 1 = \frac{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right)}{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right) - \frac{1-\alpha}{\alpha}\bB_k},
\end{align*}
which in turn yield that
\begin{align*}
    \frac{\bB_k}{\bB_j} &= \frac{\bA_k}{\bA_j} \left(\frac{1-\alpha}{\alpha}\bB_k + 1\right) \left(\frac{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right) - \frac{1-\alpha}{\alpha}\bB_k}{\frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1\right)} \right) \\
    &= \frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1 \right) - \frac{1 - \alpha}{\alpha}\bB_k.
\end{align*}
Now, observe that $0 = \alpha - \left( \left(\frac{\bB_k}{\bB_j} - \frac{\bA_k}{\bA_j} \right) \frac{\bA_j}{\bB_k (\bA_k - \bA_j)} + 1\right)^\inv$ yield that
\begin{align*}
    \frac{\bB_k}{\bB_j} &= \frac{1 - \alpha}{\alpha} \frac{\bB_k(\bA_k- \bA_j)}{\bA_j} + \frac{\bA_k}{\bA_j} = \frac{\bA_k}{\bA_j}\left(\frac{1-\alpha}{\alpha}\bB_k + 1 \right) - \frac{1 - \alpha}{\alpha}\bB_k.
\end{align*}
Thus, similar calculations with $>$ and $<$ instead of $=$, completes the claim.
\end{proof}

\begin{theorem}
Fix $\tau \geq 2$, $\lambda > 0$ and $\alpha^{(2)}, \dots, \alpha^{(\tau-1)} \in \R$, then
\begin{align*}
    \alpha^{\star(\tau)} &= \argmin_{\alpha^{(\tau)} \in \R} \norm{\tilde{\by} - f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})}_2^2 \\
    &= \frac{\left(\frac{\partial}{\partial \alpha^{(\tau)}} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})\right)^\trans \left(\tilde{\by} - \tilde{\by}^{(1)}\right)}{\norm{\frac{\partial}{\partial \alpha^{(\tau)}} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})}^2} + 1, \\
    &= 1 - \frac{\left(\tilde{\by}^{(\tau)}_{\alpha=0} - \tilde{\by}^{(1)}\right)^\trans \left(\tilde{\by} - \tilde{\by}^{(1)}\right)}{\norm{\tilde{\by}^{(\tau)}_{\alpha=0} - \tilde{\by}^{(1)}}_2^2}
\end{align*}
where $\tilde{\by}^{(1)} = f(\tilde{\bX}, \hat{\bbeta}^{(1)})$, and $\tilde{\by}^{(\tau)}_{\alpha=0} = f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}_{\alpha=0})$.
\end{theorem}
\begin{proof}
Let $\L(\alpha^{(\tau)}, \lambda) = \norm{\tilde{\by} - f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})}^2$, where $f$ depends on $\alpha^{(\tau)}$ and $\lambda$ through $\hat{\bbeta}^{(\tau)}$. Note that,
\begin{align*}
    f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) &= \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\left( \alpha^{(\tau)}\by + (1-\alpha^{(\tau)})\by^{(\tau-1)} \right) \\
    \frac{\partial}{\partial \alpha^{(\tau)}} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) &= \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\left(\by - \by^{(\tau-1)} \right).
\end{align*}
Then for fixed $\lambda > 0$, we have that
\begin{align*}
    \frac{\partial}{\partial \alpha^{(\tau)}}\L(\alpha, \lambda) &= \left(\frac{\partial}{\partial \alpha^{(\tau)}}f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) \right)^\trans \left( 2 f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) - 2\tilde{\by} \right)
\end{align*}
and since we can decompose $f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})$ as
\begin{align*}
    f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) &= \alpha^{(\tau)}\kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\left(\by - \by^{(\tau-1)} \right) + \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\by^{(\tau-1)} \\
    &= \alpha^{(\tau)}\frac{\partial}{\partial \alpha^{(\tau)}}f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) + \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\by^{(\tau-1)},
\end{align*}
and set $\frac{\partial}{ \partial \alpha^{(\tau)}}\L(\alpha^{(\tau)}, \lambda) = 0$, we can solve as follows
\begin{align*}
    \left(\partial f^{(\tau)}\right)^\trans \tilde{\by} - \left(\partial f^{(\tau)}\right)^\trans \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\by^{(\tau-1)} &= \alpha^{(\tau)} \left(\partial f^{(\tau)}\right)^\trans \left(\partial f^{(\tau)}\right) \\
    &= \alpha^{(\tau)} \norm{\partial f^{(\tau)}}^2,
\end{align*}
where we use the notation $\partial f^{(\tau)} \eqdef \frac{\partial}{\partial \alpha^{(\tau)}}f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})$ for brevity. Now since
\begin{align*}
    -\kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\by^{(\tau-1)} &= \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}(\by - \by^{(\tau-1)}) - \kappa(\tilde{\bX}, \bX)(\bK +\lambda\bI)^{-1}\by,
\end{align*}
we can finalize the proof with
\begin{align*}
    \alpha^{\star (\tau)} &= \frac{\left(\frac{\partial}{\partial \alpha} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})\right)^\trans \left(\tilde{\by} - \tilde{\by}^{(1)}\right)}{\norm{\frac{\partial}{\partial \alpha} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)})}^2} + 1,
\end{align*}
and noting that $\frac{\partial}{\partial \alpha^{(\tau)}} f(\tilde{\bX}, \hat{\bbeta}^{(\tau)}) = \tilde{\by}^{(1)} - \tilde{\by}^{(\tau)}_{\alpha=0}$.
\end{proof}


Note, in the following we state and prove a slightly more general result than Theorem \ref{thm:kernel_limit}.
\begin{theorem}
Let $\by^{(\tau)}, \hat{\bbeta}^{(\tau)}$, and $f(\cdot, \hat{\bbeta}^{(\tau)})$ be defined as above, and $\alpha \in [0,1]$, then the following limits hold
\begin{align*}
    \by^{(\infty)} &\eqdef \lim_{\tau \to \infty} \by^{(\tau)} = \alpha \bK\left(\alpha\bK + \lambda\bI_n \right)^{-1}\by \\
    f(\bx, \hat{\bbeta}^{(\infty)}) &\eqdef \lim_{\tau \to \infty} f(\bx, \hat{\bbeta}^{(\tau)}) = \alpha \kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv \left(\bI_n + (1-\alpha)\bK(\alpha\bK + \lambda\bI_n)^\inv \right)\by
\end{align*}
and if $\alpha > 0$, then
\begin{align*}
    \by^{(\infty)} &= \bK\left(\bK + \frac{\lambda}{\alpha}\bI_n \right)^{-1} \by \\
    f(\bx, \hat{\bbeta}^{(\infty)}) &= \alpha f(\bx, \hat{\bbeta}^{(1)}) + (1-\alpha)f(\bx, \hat{\bgamma}^{(\infty)})
\end{align*}
where \eqref{eq:Y_limit} corresponds to \emph{classical} kernel ridge regression with amplified regularization parameter $\frac{\lambda}{\alpha}$, and we let $\hat{\bgamma}^{(\infty)}$ denote the kernel ridge regression parameter associated with solving another kernel ridge regression on the targets $\by^{(\infty)}$ with regularization parameter $\lambda$. Furthermore, the convergence $\lim_{\tau \to \infty} \by^{(\tau)}$ is of linear rate.
\end{theorem}
\begin{proof}
By \eqref{eq:kernel_with_SVD} we have that $\bK(\bK + \lambda\bI_n)^{-1} = \bV \bD \left(\bD + \lambda\bI_n\right)^{-1}\bV^\trans$ where $\lambda > 0$, $\bD$ is positive diagonal and $\bV$ is orthogonal, and hence, the eigenvalues of $\bK(\bK + \lambda\bI_n)^{-1}$ are all smaller than $1$ in absolute value, and thus $(1-\alpha)^{\tau-1}\left(\bK(\bK + \lambda\bI_n)^\inv \right)^{\tau}$ converge to the zero-matrix when $\tau \to \infty$. Thus, using the limit for a geometric series of matrices we get that
\begin{align*}
    \lim_{\tau \to \infty} \by^{(\tau)} &= \left( \frac{\alpha}{1-\alpha} \sum_{i=1}^\infty \left((1-\alpha) \bK(\bK + \lambda\bI_n)^\inv \right)^i \right)\by \\
    &= \frac{\alpha}{1-\alpha}(1-\alpha)\bK(\bK + \lambda\bI_n)^\inv (\bI_n - (1-\alpha) \bK(\bK + \lambda\bI_n)^\inv)^\inv \by \\
    &= \alpha \bK \left(\alpha\bK + \lambda\bI_n \right)^\inv \by.
\end{align*}
If $\alpha > 0$, the remaining result for $\lim_{\tau \to \infty} \by^{(\tau)}$ follows directly. Now, by inserting $\by^{(\infty)}$ and manipulating the result, we get that
\begin{align*}
    f(\bx, \bbeta^{(\infty)}) &= \kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\alpha \by + (1-\alpha)\by^{(\infty)} \right) \\
    &= \kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\alpha \bI_n + (1-\alpha)\alpha \bK\left(\alpha\bK + \lambda\bI_n \right)^{-1} \right)\by \\
    &= \alpha\kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv\left(\bI_n + (1-\alpha)\bK\left(\alpha\bK + \lambda\bI_n \right)^{-1} \right)\by,
\end{align*}
and if $\alpha > 0$, then
\begin{align*}
    f(\bx, \bbeta^{(\infty)}) &= \alpha f(\bx, \bbeta^{(1)}) + (1-\alpha)\kappa(\bx, \bX)^\trans(\bK + \lambda\bI_n)^\inv\bK\left(\bK + \frac{\lambda}{\alpha}\bI_n \right)^{-1}\by \\
    &= \alpha f(\bx, \bbeta^{(1)}) + (1-\alpha)f(\bx, \hat{\bgamma}^{(\infty)}),
\end{align*}
where we let $\hat{\bgamma}^{(\infty)}$ denote the kernel ridge regression parameter associated with the classical kernel ridge regression problem on the targets $\by^{(\infty)}$ with regularization parameter $\lambda$.

Finally, denote by $\bC \eqdef (1-\alpha) \bK(\bK + \lambda\bI_n)^\inv$, then we have that
\begin{align*}
    \bE(t) &\eqdef \sum_{i=1}^{t} \bC^i - \sum_{i=1}^{\infty} \bC^i =  \bC^{t+1}\left(\bC - \bI_n\right)^{-1},
\end{align*}
and thus for an additional $s$ steps we have $\bE(t + s) = \bC^{t+s+1}(\bC - \bI_n)^{-1} = \bC^{s}\bE(t)$. Hence, the convergence is of linear rate as claimed.
\end{proof}
